Semantically-Aware Strategies for Stereo-Visual Robotic Obstacle Avoidance

Mobile robots in unstructured, mapless environments must rely on an obstacle avoidance module to navigate safely. The standard avoidance techniques estimate the locations of obstacles with respect to the robot but are unaware of the obstacles' identities. Consequently, the robot cannot take advantage of semantic information about obstacles when making decisions about how to navigate. We propose an obstacle avoidance module that combines visual instance segmentation with a depth map to classify and localize objects in the scene. The system avoids obstacles differentially, based on the identity of the objects: for example, the system is more cautious in response to unpredictable objects such as humans. The system can also navigate closer to harmless obstacles and ignore obstacles that pose no collision danger, enabling it to navigate more efficiently. We validate our approach in two simulated environments: one terrestrial and one underwater. Results indicate that our approach is feasible and can enable more efficient navigation strategies.

==> algs/alg1.tex <==
\begin{algorithm}[ht!]
\SetKw{KwBy}{by}
\SetKw{KwAnd}{and}

\SetAlgoLined
\tcc{Variables}
$N$ = Number of Detections \\
Avg = Avg(Depth map in Mask[i]) \\
Med = Median(Depth map) \\
\tcc{------------------------------}
\For{$i\gets0$ \KwTo N}{
\If{$p$(Detection[i]) $\geq$ $0.8$ \KwAnd Avg $\leq$ 0.8 $\times$ Med}{
% \If{Avg(Depth map in Mask[i]) $\leq$ 0.8 $\times$ Median(Depth map) }{
Depthmap = Depthmap$\times$(1-Mask[i]) \\+ Med $\times$ Mask[i] 
% }
}
}
 \caption{Depth Map Enhancement}
\label{alg:depth}
\end{algorithm}


==> figs/alg1.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Circle [id:dp2975604611520781] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (58,127.75) .. controls (58,95.03) and (84.53,68.5) .. (117.25,68.5) .. controls (149.97,68.5) and (176.5,95.03) .. (176.5,127.75) .. controls (176.5,160.47) and (149.97,187) .. (117.25,187) .. controls (84.53,187) and (58,160.47) .. (58,127.75) -- cycle ;
%Shape: Star [id:dp5613864985755701] 
\draw   (38.13,260.92) -- (39.63,264.07) -- (43,264.57) -- (40.56,267.03) -- (41.14,270.49) -- (38.13,268.85) -- (35.11,270.49) -- (35.69,267.03) -- (33.25,264.57) -- (36.62,264.07) -- cycle ;
%Shape: Star [id:dp30953777208643185] 
\draw   (247.13,22.42) -- (248.63,25.57) -- (252,26.07) -- (249.56,28.53) -- (250.14,31.99) -- (247.13,30.35) -- (244.11,31.99) -- (244.69,28.53) -- (242.25,26.07) -- (245.62,25.57) -- cycle ;
%Straight Lines [id:da5303110613173141] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (114.55,126.45) -- (67.45,103.8) ;
\draw [shift={(64.75,102.5)}, rotate = 385.69] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(117.25,127.75)}, rotate = 205.69] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da25614391267748915] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=0.63 ]   (38.13,266.21) -- (245.15,29.97) ;
\draw [shift={(247.13,27.71)}, rotate = 491.23] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.63 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Star [id:dp5675693409434179] 
\draw   (61.86,233.22) -- (63.36,236.37) -- (66.73,236.87) -- (64.3,239.33) -- (64.87,242.79) -- (61.86,241.15) -- (58.85,242.79) -- (59.42,239.33) -- (56.98,236.87) -- (60.35,236.37) -- cycle ;
%Shape: Star [id:dp1004239479943716] 
\draw   (85.06,206.82) -- (86.56,209.97) -- (89.93,210.47) -- (87.5,212.93) -- (88.07,216.39) -- (85.06,214.75) -- (82.05,216.39) -- (82.62,212.93) -- (80.18,210.47) -- (83.55,209.97) -- cycle ;
%Shape: Star [id:dp32673265657973816] 
\draw   (108.26,181.62) -- (109.76,184.77) -- (113.13,185.27) -- (110.7,187.73) -- (111.27,191.19) -- (108.26,189.55) -- (105.25,191.19) -- (105.82,187.73) -- (103.38,185.27) -- (106.75,184.77) -- cycle ;
%Shape: Star [id:dp8122524493934715] 
\draw   (174.26,106.02) -- (175.76,109.17) -- (179.13,109.67) -- (176.7,112.13) -- (177.27,115.59) -- (174.26,113.95) -- (171.25,115.59) -- (171.82,112.13) -- (169.38,109.67) -- (172.75,109.17) -- cycle ;
%Shape: Star [id:dp9934033956713975] 
\draw   (196.26,79.22) -- (197.76,82.37) -- (201.13,82.87) -- (198.7,85.33) -- (199.27,88.79) -- (196.26,87.15) -- (193.25,88.79) -- (193.82,85.33) -- (191.38,82.87) -- (194.75,82.37) -- cycle ;
%Shape: Star [id:dp24423428627288502] 
\draw   (218.66,54.02) -- (220.16,57.17) -- (223.53,57.67) -- (221.1,60.13) -- (221.67,63.59) -- (218.66,61.95) -- (215.65,63.59) -- (216.22,60.13) -- (213.78,57.67) -- (217.15,57.17) -- cycle ;
%Shape: Star [id:dp7211968231635728] 
\draw   (175.06,139.62) -- (176.56,142.77) -- (179.93,143.27) -- (177.5,145.73) -- (178.07,149.19) -- (175.06,147.55) -- (172.05,149.19) -- (172.62,145.73) -- (170.18,143.27) -- (173.55,142.77) -- cycle ;
%Flowchart: Summing Junction [id:dp40596458450252415] 
\draw   (112.05,127.75) .. controls (112.05,130.62) and (114.38,132.95) .. (117.25,132.95) .. controls (120.12,132.95) and (122.45,130.62) .. (122.45,127.75) .. controls (122.45,124.88) and (120.12,122.55) .. (117.25,122.55) .. controls (114.38,122.55) and (112.05,124.88) .. (112.05,127.75) -- cycle ; \draw   (113.57,131.43) -- (120.93,124.07) ; \draw   (120.93,131.43) -- (113.57,124.07) ;
%Shape: Star [id:dp4659134265621454] 
\draw   (149.46,171.22) -- (150.96,174.37) -- (154.33,174.87) -- (151.9,177.33) -- (152.47,180.79) -- (149.46,179.15) -- (146.45,180.79) -- (147.02,177.33) -- (144.58,174.87) -- (147.95,174.37) -- cycle ;
%Straight Lines [id:da29670193779713294] 
\draw    (175.65,145.09) -- (156.04,138.21) ;
\draw [shift={(153.2,137.22)}, rotate = 379.32] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da8925668240747111] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ]   (175.65,145.09) -- (183.4,123) ;
\draw [shift={(184.39,120.17)}, rotate = 469.32] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da3108812027682837] 
\draw    (108.12,187.07) -- (113.62,167.02) ;
\draw [shift={(114.41,164.13)}, rotate = 465.35] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da1317741725519319] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ]   (108.12,187.07) -- (121.64,171.47) ;
\draw [shift={(123.6,169.2)}, rotate = 490.91] [fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da15876093811427872] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ]   (108.12,187.07) -- (130.69,193.26) ;
\draw [shift={(133.58,194.06)}, rotate = 195.35] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da644761124320866] 
\draw    (150.02,177.78) -- (139.09,164.33) ;
\draw [shift={(137.2,162)}, rotate = 410.90999999999997] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da4900642840068008] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ]   (150.02,177.78) -- (168.54,163.47) ;
\draw [shift={(170.92,161.63)}, rotate = 502.32] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da3547814878124329] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ]   (149.46,176.51) -- (162.98,160.91) ;
\draw [shift={(164.94,158.64)}, rotate = 490.91] [fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7531330869094726] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ]   (175.06,144.91) -- (188.58,129.31) ;
\draw [shift={(190.54,127.04)}, rotate = 490.91] [fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da5478161461914619] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ]   (38.13,266.21) -- (52.85,249.08) ;
\draw [shift={(54.8,246.8)}, rotate = 490.67] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da13965634958186657] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ]   (61.86,238.51) -- (76.58,221.38) ;
\draw [shift={(78.53,219.1)}, rotate = 490.67] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da48599417157163405] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ]   (85.06,212.11) -- (99.78,194.98) ;
\draw [shift={(101.73,192.7)}, rotate = 490.67] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da5297815646917878] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ]   (174.26,111.31) -- (188.98,94.18) ;
\draw [shift={(190.93,91.9)}, rotate = 490.67] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da4995421315760966] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ]   (196.7,85.33) -- (211.42,68.19) ;
\draw [shift={(213.37,65.92)}, rotate = 490.67] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da1739575760414318] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ]   (218.66,60.31) -- (233.38,43.18) ;
\draw [shift={(235.33,40.9)}, rotate = 490.67] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (119.5,108.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {O};
% Text Node
\draw (14.5,253) node [anchor=north west][inner sep=0.75pt]   [align=left] {R};
% Text Node
\draw (224.5,15) node [anchor=north west][inner sep=0.75pt]   [align=left] {G};
% Text Node
\draw (79,107.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {d{\scriptsize 0}};


\end{tikzpicture}


==> figs/pipeline.tex <==
\begin{figure*}
    \centering

% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
% %uncomment if require: \path (0,660); %set diagram left start at 0, and has height of 660

% %Image [id:dp4117624803164248] 
% \draw (107.75,178.78) node  {\includegraphics[width=139.13pt,height=52.17pt]{imgs/sidebyside_00541.jpg}};
% %Image [id:dp4743686419266042] 
% \draw (61.83,66) node  {\includegraphics[width=70pt,height=52.5pt]{imgs/frame_left_000541.png}};
% %Image [id:dp851680704866115] 
% \draw (155.17,66) node  {\includegraphics[width=70pt,height=52.5pt]{imgs/frame_right_000541.png}};
% %Image [id:dp4627256015601149] 
% \draw (287.08,110.06) node  {\includegraphics[width=73.88pt,height=55.41pt]{imgs/left_rect_00541.jpg}};
% %Image [id:dp8992006466247122] 
% \draw (287.17,184) node  {\includegraphics[width=74pt,height=55.5pt]{imgs/disparity_00541.jpg}};
% %Image [id:dp7211936204042146] 
% \draw (527.25,146.44) node  {\includegraphics[width=172.88pt,height=129.66pt]{imgs/left_inst_00541.png}};
% %Straight Lines [id:da6117107806396676] 
% \draw    (108.5,101) -- (108.5,139) ;
% \draw [shift={(108.5,142)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Shape: Rectangle [id:dp7736292424689921] 
% \draw   (5,24) -- (345.5,24) -- (345.5,269) -- (5,269) -- cycle ;
% %Image [id:dp6852259717181188] 
% \draw (142.42,373.63) node  {\includegraphics[width=126.88pt,height=95.16pt]{imgs/enhanced_color_00541.jpg}};
% %Image [id:dp5849376129751944] 
% \draw (144.47,563.5) node  {\includegraphics[width=175.45pt,height=120.75pt]{imgs/masked_buffer_00541.jpg}};
% %Image [id:dp6254287432701746] 
% \draw (548.67,373.5) node  {\includegraphics[width=127pt,height=95.25pt]{imgs/before_00541.jpg}};
% %Image [id:dp0003503984543555827] 
% \draw (421.75,342.37) node  {\includegraphics[width=63.38pt,height=48.56pt]{imgs/crop_before0_00541.jpg}};
% %Image [id:dp9642838841336003] 
% \draw (269.42,342.5) node  {\includegraphics[width=63.62pt,height=48.75pt]{imgs/crop_after0_00541.jpg}};
% %Image [id:dp363456638869323] 
% \draw (421.75,405.23) node  {\includegraphics[width=63.38pt,height=47.19pt]{imgs/crop_before1_00541.jpg}};
% %Image [id:dp8326232479795599] 
% \draw (269.5,405.42) node  {\includegraphics[width=63.75pt,height=47.47pt]{imgs/crop_after1_00541.jpg}};
% %Shape: Rectangle [id:dp3065549942703125] 
% \draw   (399,23) -- (656,23) -- (656,268) -- (399,268) -- cycle ;
% %Shape: Rectangle [id:dp5437537033260673] 
% \draw   (10,304) -- (653,304) -- (653,446) -- (10,446) -- cycle ;
% %Right Arrow [id:dp13691759988412366] 
% \draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (354,139) -- (379.8,139) -- (379.8,134) -- (397,144) -- (379.8,154) -- (379.8,149) -- (354,149) -- cycle ;
% %Curve Lines [id:da6103396021438428] 
% \draw    (108.5,215) .. controls (123.85,245.69) and (215.15,261.68) .. (280.04,225.12) ;
% \draw [shift={(282,224)}, rotate = 509.69] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Shape: Rectangle [id:dp02540138902453415] 
% \draw   (10.5,477) -- (277,477) -- (277,649) -- (10.5,649) -- cycle ;
% %Right Arrow [id:dp01269905030609264] 
% \draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (529.38,271) -- (529.38,288.1) -- (534.5,288.1) -- (524.25,299.5) -- (514,288.1) -- (519.13,288.1) -- (519.13,271) -- cycle ;
% %Straight Lines [id:da2920455814323397] 
% \draw    (369,376) -- (327.5,376) ;
% \draw [shift={(324.5,376)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Image [id:dp6065472379451662] 
% \draw (502.5,563.13) node  {\includegraphics[width=164.25pt,height=123.19pt]{imgs/targetsrgb00541.jpg}};
% %Shape: Rectangle [id:dp6322302523893162] 
% \draw   (369.5,477) -- (636,477) -- (636,649) -- (369.5,649) -- cycle ;
% %Right Arrow [id:dp016762234412186716] 
% \draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (302,551) -- (327.8,551) -- (327.8,546) -- (345,556) -- (327.8,566) -- (327.8,561) -- (302,561) -- cycle ;
% %Right Arrow [id:dp12754474043695696] 
% \draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (233.75,451.3) -- (233.75,464.34) -- (239,464.34) -- (228.5,473.02) -- (218,464.34) -- (223.25,464.34) -- (223.25,451.3) -- cycle ;

% % Text Node
% \draw (60,121) node   [align=left] {Rectification};
% % Text Node
% \draw (69,238) node   [align=left] {Disparity \\Calculation};
% % Text Node
% \draw (66,10) node   [align=left] {\textit{Depth Estimation}};
% % Text Node
% \draw (501,10) node   [align=left] {\textit{Instance Segmentation with Depth map}};
% % Text Node
% \draw (82,292) node   [align=left] {\textit{Depth Enhancement}};
% % Text Node
% \draw (103,465) node   [align=left] {\textit{Masks Update with Buffers}};
% % Text Node
% \draw (450,466) node   [align=left] {\textit{Decision for Exploration}};
% \end{tikzpicture}

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,660); %set diagram left start at 0, and has height of 660

%Image [id:dp4117624803164248] 
\draw (109.5,146.5) node  {\includegraphics[width=122pt,height=45.75pt]{imgs/sidebyside_00541.jpg}};
%Image [id:dp4743686419266042] 
\draw (67.83,61.5) node  {\includegraphics[width=61pt,height=45.75pt]{imgs/frame_left_000541.png}};
%Image [id:dp851680704866115] 
\draw (149.17,61.5) node  {\includegraphics[width=61pt,height=45.75pt]{imgs/frame_right_000541.png}};
%Image [id:dp8992006466247122] 
\draw (313.5,61.5) node  {\includegraphics[width=61pt,height=45.75pt]{imgs/disparity_00541.jpg}};
%Image [id:dp7211936204042146] 
\draw (534.5,103.5) node  {\includegraphics[width=147pt,height=110.25pt]{imgs/test541_2.jpg}};
%Straight Lines [id:da6117107806396676] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (108.5,92) -- (108.5,111) ;
\draw [shift={(108.5,114)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp7736292424689921] 
\draw   (19,24) -- (641.5,24) -- (641.5,186) -- (19,186) -- cycle ;
%Image [id:dp6852259717181188] 
\draw (550.58,280.81) node  {\includegraphics[width=126.88pt,height=95.16pt]{imgs/enhanced_color_00541.jpg}};
%Image [id:dp5849376129751944] 
\draw (133.64,458.5) node  {\includegraphics[width=160.2pt,height=110.25pt]{imgs/masked_buffer_00541.jpg}};
%Image [id:dp6254287432701746] 
\draw (110.83,281.5) node  {\includegraphics[width=127pt,height=95.25pt]{imgs/before_00541.jpg}};
%Image [id:dp0003503984543555827] 
\draw (237.75,250.37) node  {\includegraphics[width=63.38pt,height=48.56pt]{imgs/crop_before0_00541.jpg}};
%Image [id:dp9642838841336003] 
\draw (423.58,249.87) node  {\includegraphics[width=63.62pt,height=48.75pt]{imgs/crop_after0_00541.jpg}};
%Image [id:dp363456638869323] 
\draw (237.75,314.21) node  {\includegraphics[width=63.38pt,height=47.19pt]{imgs/crop_before1_00541.jpg}};
%Image [id:dp8326232479795599] 
\draw (423.5,314.02) node  {\includegraphics[width=63.75pt,height=47.47pt]{imgs/crop_after1_00541.jpg}};
%Shape: Rectangle [id:dp5437537033260673] 
\draw   (18,212) -- (642.5,212) -- (642.5,354) -- (18,354) -- cycle ;
%Right Arrow [id:dp01269905030609264] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (343.63,190) -- (343.63,200.2) -- (354.5,200.2) -- (332.75,207) -- (311,200.2) -- (321.88,200.2) -- (321.88,190) -- cycle ;
%Straight Lines [id:da2920455814323397] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (282.5,254) -- (373.5,254) ;
\draw [shift={(376.5,254)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Image [id:dp6065472379451662] 
\draw (537.44,457.5) node  {\includegraphics[width=147pt,height=110.25pt]{imgs/targetsrgb00541.jpg}};
%Straight Lines [id:da4830595390808743] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (191.83,115) -- (268.01,63.68) ;
\draw [shift={(270.5,62)}, rotate = 506.03] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Image [id:dp35073585442049704] 
\draw (314.83,146.5) node  {\includegraphics[width=61pt,height=45.75pt]{imgs/col_seg_541.jpg}};
%Straight Lines [id:da655941522841847] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (194.5,138) -- (272.5,138) ;
\draw [shift={(275.5,138)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw  [dash pattern={on 4.5pt off 4.5pt}] (313,91) .. controls (321.33,97.94) and (329.67,102.11) .. (338,103.5) .. controls (329.67,104.89) and (321.33,109.06) .. (313,116) ;
%Straight Lines [id:da8552304865530553] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (337.5,104) -- (428.5,104) ;
\draw [shift={(431.5,104)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da3047090904503069] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (283,315) -- (373.5,315) ;
\draw [shift={(376.5,315)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp49729217230614453] 
\draw   (20,377) -- (642.5,377) -- (642.5,539) -- (20,539) -- cycle ;
%Right Arrow [id:dp002459240460149781] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (344.63,357) -- (344.63,367.2) -- (355.5,367.2) -- (333.75,374) -- (312,367.2) -- (322.88,367.2) -- (322.88,357) -- cycle ;
%Straight Lines [id:da45638313627088545] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (244,458) -- (431.5,458) ;
\draw [shift={(434.5,458)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp7061733350365929] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=1.5]  (24,27) -- (193.5,27) -- (193.5,95.29) -- (24,95.29) -- cycle ;
%Shape: Rectangle [id:dp7800006580393155] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]  (435.5,381) -- (639.5,381) -- (639.5,535) -- (435.5,535) -- cycle ;

% Text Node
\draw (66,105) node  [font=\footnotesize] [align=left] {Rectification};
% Text Node
\draw (78,12) node   [align=left] {\textit{Depth Estimation}};
% Text Node
\draw (80,197) node   [align=left] {\textit{Depth Enhancement}};
% Text Node
\draw (100,364) node   [align=left] {\textit{Masks Update with Buffers}};
% Text Node
\draw (559,363) node   [align=left] {\textit{Decision for Exploration}};
% Text Node
\draw (233,64) node  [font=\footnotesize,rotate=-327.47] [align=left] {Disparity\\Calculation};
% Text Node
\draw (232,158) node  [font=\footnotesize] [align=left] {Instance\\Segmentation};
% Text Node
\draw (394,123) node  [font=\footnotesize] [align=left] {Combine};
% Text Node
\draw (505,11) node   [align=left] {\textit{Instance Segmentation with Depth Information}};
% Text Node
\draw (213,33) node  [font=\footnotesize,color={rgb, 255:red, 0; green, 48; blue, 255 }  ,opacity=1 ] [align=left] {\textbf{\underline{Input}}};
% Text Node
\draw (412,388) node  [font=\footnotesize,color={rgb, 255:red, 0; green, 48; blue, 255 }  ,opacity=1 ] [align=left] {\textcolor[rgb]{1,0,0}{\underline{\textbf{Output}}}};


\end{tikzpicture}



\caption{Illustration of our pipeline to decide where to explore from a pair of stereo images. Input and output are marked with ``blue''  and ``red'' color respectively.}
\label{fig:pipeline}
\vspace{-4mm}
\end{figure*}














% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
% %uncomment if require: \path (0,660); %set diagram left start at 0, and has height of 660

% %Image [id:dp4117624803164248] 
% \draw (107.75,178.78) node  {\includegraphics[width=139.13pt,height=52.17pt]{imgs/sidebyside_00541.jpg}};
% %Image [id:dp4743686419266042] 
% \draw (61.83,66) node  {\includegraphics[width=70pt,height=52.5pt]{imgs/frame_left_000541.png}};
% %Image [id:dp851680704866115] 
% \draw (155.17,66) node  {\includegraphics[width=70pt,height=52.5pt]{imgs/frame_right_000541.png}};
% %Image [id:dp4627256015601149] 
% \draw (287.08,110.06) node  {\includegraphics[width=73.88pt,height=55.41pt]{imgs/left_rect_00541.jpg}};
% %Image [id:dp8992006466247122] 
% \draw (287.17,184) node  {\includegraphics[width=74pt,height=55.5pt]{imgs/disparity_00541.jpg}};
% %Image [id:dp7211936204042146] 
% \draw (527.25,146.44) node  {\includegraphics[width=172.88pt,height=129.66pt]{imgs/left_inst_00541.png}};
% %Straight Lines [id:da6117107806396676] 
% \draw    (108.5,101) -- (108.5,139) ;
% \draw [shift={(108.5,142)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Shape: Rectangle [id:dp7736292424689921] 
% \draw   (5,24) -- (345.5,24) -- (345.5,269) -- (5,269) -- cycle ;
% %Image [id:dp6852259717181188] 
% \draw (142.42,373.63) node  {\includegraphics[width=126.88pt,height=95.16pt]{imgs/enhanced_color_00541.jpg}};
% %Image [id:dp5849376129751944] 
% \draw (144.47,563.5) node  {\includegraphics[width=175.45pt,height=120.75pt]{imgs/masked_buffer_00541.jpg}};
% %Image [id:dp6254287432701746] 
% \draw (548.67,373.5) node  {\includegraphics[width=127pt,height=95.25pt]{imgs/before_00541.jpg}};
% %Image [id:dp0003503984543555827] 
% \draw (421.75,342.37) node  {\includegraphics[width=63.38pt,height=48.56pt]{imgs/crop_before0_00541.jpg}};
% %Image [id:dp9642838841336003] 
% \draw (269.42,342.5) node  {\includegraphics[width=63.62pt,height=48.75pt]{imgs/crop_after0_00541.jpg}};
% %Image [id:dp363456638869323] 
% \draw (421.75,405.23) node  {\includegraphics[width=63.38pt,height=47.19pt]{imgs/crop_before1_00541.jpg}};
% %Image [id:dp8326232479795599] 
% \draw (269.5,405.42) node  {\includegraphics[width=63.75pt,height=47.47pt]{imgs/crop_after1_00541.jpg}};
% %Shape: Rectangle [id:dp3065549942703125] 
% \draw   (399,23) -- (656,23) -- (656,268) -- (399,268) -- cycle ;
% %Shape: Rectangle [id:dp5437537033260673] 
% \draw   (10,304) -- (653,304) -- (653,446) -- (10,446) -- cycle ;
% %Right Arrow [id:dp13691759988412366] 
% \draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (354,139) -- (379.8,139) -- (379.8,134) -- (397,144) -- (379.8,154) -- (379.8,149) -- (354,149) -- cycle ;
% %Curve Lines [id:da6103396021438428] 
% \draw    (108.5,215) .. controls (123.85,245.69) and (215.15,261.68) .. (280.04,225.12) ;
% \draw [shift={(282,224)}, rotate = 509.69] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Shape: Rectangle [id:dp02540138902453415] 
% \draw   (10.5,477) -- (277,477) -- (277,649) -- (10.5,649) -- cycle ;
% %Right Arrow [id:dp01269905030609264] 
% \draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (529.38,271) -- (529.38,288.1) -- (534.5,288.1) -- (524.25,299.5) -- (514,288.1) -- (519.13,288.1) -- (519.13,271) -- cycle ;
% %Straight Lines [id:da2920455814323397] 
% \draw    (369,376) -- (327.5,376) ;
% \draw [shift={(324.5,376)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Image [id:dp6065472379451662] 
% \draw (502.5,563.13) node  {\includegraphics[width=164.25pt,height=123.19pt]{imgs/targetsrgb00541.jpg}};
% %Shape: Rectangle [id:dp6322302523893162] 
% \draw   (369.5,477) -- (636,477) -- (636,649) -- (369.5,649) -- cycle ;
% %Right Arrow [id:dp016762234412186716] 
% \draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (302,551) -- (327.8,551) -- (327.8,546) -- (345,556) -- (327.8,566) -- (327.8,561) -- (302,561) -- cycle ;
% %Right Arrow [id:dp12754474043695696] 
% \draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (233.75,451.3) -- (233.75,464.34) -- (239,464.34) -- (228.5,473.02) -- (218,464.34) -- (223.25,464.34) -- (223.25,451.3) -- cycle ;

% % Text Node
% \draw (60,121) node   [align=left] {Rectification};
% % Text Node
% \draw (69,238) node   [align=left] {Disparity \\Calculation};
% % Text Node
% \draw (66,10) node   [align=left] {\textit{Depth Estimation}};
% % Text Node
% \draw (501,10) node   [align=left] {\textit{Instance Segmentation with Depth map}};
% % Text Node
% \draw (82,292) node   [align=left] {\textit{Depth Enhancement}};
% % Text Node
% \draw (103,465) node   [align=left] {\textit{Masks Update with Buffers}};
% % Text Node
% \draw (450,466) node   [align=left] {\textit{Decision for Exploration}};
% \end{tikzpicture}

==> figs/pipelinenew.tex <==
\begin{figure*}
    \centering





\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.8pt,y=0.8pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,347); %set diagram left start at 0, and has height of 347

%Image [id:dp7877209410508317] 
\draw (66.67,210.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/frame_left_000541.png}};
%Image [id:dp6669996382057675] 
\draw (156,210.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/frame_right_000541.png}};
%Image [id:dp872431748781199] 
\draw (112.33,302.5) node  {\includegraphics[width=134pt,height=50.25pt]{imgs/sidebyside_00541.jpg}};
%Image [id:dp6532056361386971] 
\draw (317.33,210.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/disparity_00541.jpg}};
%Image [id:dp9145691484847331] 
\draw (318.33,302.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/col_seg_541.jpg}};
%Image [id:dp5231006751651657] 
\draw (511.75,256.31) node  {\includegraphics[width=158.63pt,height=118.97pt]{imgs/test541_2.jpg}};
%Straight Lines [id:da703085077490017] 
\draw    (111.33,244) -- (111.33,267) ;
\draw [shift={(111.33,270)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da997936862257925] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (201.67,269) -- (271.21,209.94) ;
\draw [shift={(273.5,208)}, rotate = 499.66] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da8038026727180496] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (201.67,300) -- (264.5,300) ;
\draw [shift={(267.5,300)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da23986816459559224] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (339.5,257) -- (402.5,257) ;
\draw [shift={(405.5,257)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da2612641734016845] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (310.5,243) .. controls (319.5,261) and (333.5,254) .. (339.5,257) ;
%Curve Lines [id:da40991455130375476] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (312.5,269) .. controls (319.5,259) and (336.5,256) .. (339.5,257) ;
%Rounded Rect [id:dp9593613374760706] 
\draw   (15,147.17) .. controls (15,140.45) and (20.45,135) .. (27.17,135) -- (614.33,135) .. controls (621.05,135) and (626.5,140.45) .. (626.5,147.17) -- (626.5,330.83) .. controls (626.5,337.55) and (621.05,343) .. (614.33,343) -- (27.17,343) .. controls (20.45,343) and (15,337.55) .. (15,330.83) -- cycle ;
%Shape: Rectangle [id:dp3414189783321764] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=2.25]  (22,177) -- (200.67,177) -- (200.67,244) -- (22,244) -- cycle ;
%Image [id:dp8315724500453314] 
\draw (73.54,64.72) node  {\includegraphics[width=52.56pt,height=39.42pt]{imgs/frame_left_000541.png}};
%Image [id:dp17060944368797948] 
\draw (143.63,64.72) node  {\includegraphics[width=52.56pt,height=39.42pt]{imgs/frame_right_000541.png}};
%Shape: Rectangle [id:dp5411990237200444] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=2.25]  (38.5,38.44) -- (178.67,38.44) -- (178.67,91) -- (38.5,91) -- cycle ;
%Rounded Rect [id:dp8968765113790105] 
\draw   (15.5,14.33) .. controls (15.5,9.73) and (19.23,6) .. (23.83,6) -- (193.17,6) .. controls (197.77,6) and (201.5,9.73) .. (201.5,14.33) -- (201.5,90.67) .. controls (201.5,95.27) and (197.77,99) .. (193.17,99) -- (23.83,99) .. controls (19.23,99) and (15.5,95.27) .. (15.5,90.67) -- cycle ;
%Up Down Arrow [id:dp4246149856363397] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (311.5,111) -- (328.25,102) -- (345,111) -- (335,111) -- (335,122) -- (345,122) -- (328.25,131) -- (311.5,122) -- (321.5,122) -- (321.5,111) -- cycle ;
%Image [id:dp05773900655841713] 
\draw (551.86,60.5) node  {\includegraphics[width=79.28pt,height=47.25pt]{imgs/aqua.jpg}};
%Rounded Rect [id:dp8230713593534384] 
\draw   (473.17,14.33) .. controls (473.17,9.73) and (476.9,6) .. (481.5,6) -- (618.17,6) .. controls (622.77,6) and (626.5,9.73) .. (626.5,14.33) -- (626.5,90.67) .. controls (626.5,95.27) and (622.77,99) .. (618.17,99) -- (481.5,99) .. controls (476.9,99) and (473.17,95.27) .. (473.17,90.67) -- cycle ;
%Rounded Rect [id:dp8551143788810873] 
\draw   (277.17,14.33) .. controls (277.17,9.73) and (280.9,6) .. (285.5,6) -- (380.83,6) .. controls (385.44,6) and (389.17,9.73) .. (389.17,14.33) -- (389.17,90.67) .. controls (389.17,95.27) and (385.44,99) .. (380.83,99) -- (285.5,99) .. controls (280.9,99) and (277.17,95.27) .. (277.17,90.67) -- cycle ;
%Right Arrow [id:dp3117459154120561] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (401.75,50.25) -- (443.5,50.25) -- (443.5,45) -- (459.5,55.5) -- (443.5,66) -- (443.5,60.75) -- (401.75,60.75) -- cycle ;
%Right Arrow [id:dp8603749881772891] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (211.17,51.25) -- (251.65,51.25) -- (251.65,46) -- (267.17,56.5) -- (251.65,67) -- (251.65,61.75) -- (211.17,61.75) -- cycle ;

% Text Node
\draw (293,30.38) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{53.00810800000001pt}\setlength\topsep{0pt}
\begin{center}
Obstacle\\Avoidance \\Module
\end{center}

\end{minipage}};
% Text Node
\draw (200.7,230.34) node [anchor=north west][inner sep=0.75pt]  [rotate=-318.34] [align=left] {{\scriptsize Disparity}\\{\scriptsize Calculation}};
% Text Node
\draw (201.67,302) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Instance}\\{\scriptsize Segmentation}};
% Text Node
\draw (351,245) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Combine}};
% Text Node
\draw (48,249) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Rectification}};
% Text Node
\draw (204.67,172) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textcolor[rgb]{0,0.01,1}{\textbf{Input}}}};
% Text Node
\draw (22,146) node [anchor=north west][inner sep=0.75pt]   [align=left] {Instance Segmentation with Depth Information};
% Text Node
\draw (64.49,14) node [anchor=north west][inner sep=0.75pt]   [align=left] {Stereo Images};
% Text Node
\draw (26,116) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large SOAR}};
% Text Node
\draw (526.49,10) node [anchor=north west][inner sep=0.75pt]   [align=left] {Robot};


\end{tikzpicture}



% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
% %uncomment if require: \path (0,311); %set diagram left start at 0, and has height of 311

% %Image [id:dp7877209410508317] 
% \draw (67.67,92.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/frame_left_000541.png}};
% %Image [id:dp6669996382057675] 
% \draw (157,92.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/frame_right_000541.png}};
% %Image [id:dp872431748781199] 
% \draw (113.33,184.5) node  {\includegraphics[width=134pt,height=50.25pt]{imgs/sidebyside_00541.jpg}};
% %Image [id:dp6532056361386971] 
% \draw (318.33,92.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/disparity_00541.jpg}};
% %Image [id:dp9145691484847331] 
% \draw (319.33,184.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/col_seg_541.jpg}};
% %Image [id:dp5231006751651657] 
% \draw (512.75,138.31) node  {\includegraphics[width=158.63pt,height=118.97pt]{imgs/test541_2.jpg}};
% %Straight Lines [id:da703085077490017] 
% \draw    (112.33,126) -- (112.33,149) ;
% \draw [shift={(112.33,152)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Straight Lines [id:da997936862257925] 
% \draw  [dash pattern={on 4.5pt off 4.5pt}]  (202.67,151) -- (272.21,91.94) ;
% \draw [shift={(274.5,90)}, rotate = 499.66] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Straight Lines [id:da8038026727180496] 
% \draw  [dash pattern={on 4.5pt off 4.5pt}]  (202.67,182) -- (265.5,182) ;
% \draw [shift={(268.5,182)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Straight Lines [id:da23986816459559224] 
% \draw  [dash pattern={on 4.5pt off 4.5pt}]  (340.5,139) -- (403.5,139) ;
% \draw [shift={(406.5,139)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Curve Lines [id:da2612641734016845] 
% \draw  [dash pattern={on 4.5pt off 4.5pt}]  (311.5,125) .. controls (320.5,143) and (334.5,136) .. (340.5,139) ;
% %Curve Lines [id:da40991455130375476] 
% \draw  [dash pattern={on 4.5pt off 4.5pt}]  (313.5,151) .. controls (320.5,141) and (337.5,138) .. (340.5,139) ;
% %Rounded Rect [id:dp9593613374760706] 
% \draw   (16,29.26) .. controls (16,18.62) and (24.62,10) .. (35.26,10) -- (608.24,10) .. controls (618.88,10) and (627.5,18.62) .. (627.5,29.26) -- (627.5,205.74) .. controls (627.5,216.38) and (618.88,225) .. (608.24,225) -- (35.26,225) .. controls (24.62,225) and (16,216.38) .. (16,205.74) -- cycle ;
% %Rounded Rect [id:dp6835927400145065] 
% \draw   (16.5,257.6) .. controls (16.5,255.08) and (18.54,253.03) .. (21.07,253.03) -- (289.93,253.03) .. controls (292.46,253.03) and (294.5,255.08) .. (294.5,257.6) -- (294.5,299.43) .. controls (294.5,301.96) and (292.46,304) .. (289.93,304) -- (21.07,304) .. controls (18.54,304) and (16.5,301.96) .. (16.5,299.43) -- cycle ;
% %Down Arrow [id:dp7638490016860275] 
% \draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (258.22,239.14) -- (264.78,239.23) -- (281.55,225.73) -- (294.66,225.92) -- (277.9,239.42) -- (284.46,239.51) -- (253.92,253.35) -- cycle ;
% %Right Arrow [id:dp3553298079486289] 
% \draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (295.75,272.25) -- (326.2,272.25) -- (326.2,267) -- (346.5,277.5) -- (326.2,288) -- (326.2,282.75) -- (295.75,282.75) -- cycle ;
% %Shape: Rectangle [id:dp3414189783321764] 
% \draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=2.25]  (23,59) -- (201.67,59) -- (201.67,126) -- (23,126) -- cycle ;
% %Rounded Rect [id:dp3171462327119514] 
% \draw   (346.5,255.6) .. controls (346.5,253.08) and (348.54,251.03) .. (351.07,251.03) -- (619.93,251.03) .. controls (622.46,251.03) and (624.5,253.08) .. (624.5,255.6) -- (624.5,297.43) .. controls (624.5,299.96) and (622.46,302) .. (619.93,302) -- (351.07,302) .. controls (348.54,302) and (346.5,299.96) .. (346.5,297.43) -- cycle ;

% % Text Node
% \draw (95,270) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Modified APF}};
% % Text Node
% \draw (435,270) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Exploration}};
% % Text Node
% \draw (205.19,111.25) node [anchor=north west][inner sep=0.75pt]  [rotate=-318.34] [align=left] {{\scriptsize Disparity}\\{\scriptsize Calculation}};
% % Text Node
% \draw (204.67,185) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Instance}\\{\scriptsize Segmentation}};
% % Text Node
% \draw (354,124) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Combine}};
% % Text Node
% \draw (51,131) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Rectification}};
% % Text Node
% \draw (207.67,57) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textcolor[rgb]{0,0.01,1}{\textbf{Input}}}};
% % Text Node
% \draw (28,20) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Instance Segmentation with Depth Information}};


% \end{tikzpicture}

\caption{Illustration of our pipeline to decide where to explore from a pair of stereo images. Input is marked with ``blue'' color.}
\label{fig:pipeline}
\vspace{-4mm}
\end{figure*}


==> figs/pipelinenew1.tex <==
\begin{figure}
    \centering

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.8pt,y=0.8pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,347); %set diagram left start at 0, and has height of 347

%Image [id:dp7877209410508317] 
\draw (66.67,210.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/frame_left_000541.png}};
%Image [id:dp6669996382057675] 
\draw (156,210.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/frame_right_000541.png}};
%Image [id:dp872431748781199] 
\draw (112.33,302.5) node  {\includegraphics[width=134pt,height=50.25pt]{imgs/sidebyside_00541.jpg}};
%Image [id:dp6532056361386971] 
\draw (317.33,210.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/disparity_00541.jpg}};
%Image [id:dp9145691484847331] 
\draw (318.33,302.5) node  {\includegraphics[width=67pt,height=50.25pt]{imgs/col_seg_541.jpg}};
%Image [id:dp5231006751651657] 
\draw (511.75,256.31) node  {\includegraphics[width=158.63pt,height=118.97pt]{imgs/test541_2.jpg}};
%Straight Lines [id:da703085077490017] 
\draw    (111.33,244) -- (111.33,267) ;
\draw [shift={(111.33,270)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da997936862257925] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (201.67,269) -- (271.21,209.94) ;
\draw [shift={(273.5,208)}, rotate = 499.66] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da8038026727180496] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (201.67,300) -- (264.5,300) ;
\draw [shift={(267.5,300)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da23986816459559224] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (339.5,257) -- (402.5,257) ;
\draw [shift={(405.5,257)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da2612641734016845] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (310.5,243) .. controls (319.5,261) and (333.5,254) .. (339.5,257) ;
%Curve Lines [id:da40991455130375476] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (312.5,269) .. controls (319.5,259) and (336.5,256) .. (339.5,257) ;
%Rounded Rect [id:dp9593613374760706] 
\draw   (15,147.17) .. controls (15,140.45) and (20.45,135) .. (27.17,135) -- (614.33,135) .. controls (621.05,135) and (626.5,140.45) .. (626.5,147.17) -- (626.5,330.83) .. controls (626.5,337.55) and (621.05,343) .. (614.33,343) -- (27.17,343) .. controls (20.45,343) and (15,337.55) .. (15,330.83) -- cycle ;
%Shape: Rectangle [id:dp3414189783321764] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=2.25]  (22,177) -- (200.67,177) -- (200.67,244) -- (22,244) -- cycle ;
%Image [id:dp8315724500453314] 
\draw (73.54,64.72) node  {\includegraphics[width=52.56pt,height=39.42pt]{imgs/frame_left_000541.png}};
%Image [id:dp17060944368797948] 
\draw (143.63,64.72) node  {\includegraphics[width=52.56pt,height=39.42pt]{imgs/frame_right_000541.png}};
%Shape: Rectangle [id:dp5411990237200444] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=2.25]  (38.5,38.44) -- (178.67,38.44) -- (178.67,91) -- (38.5,91) -- cycle ;
%Rounded Rect [id:dp8968765113790105] 
\draw   (15.5,14.33) .. controls (15.5,9.73) and (19.23,6) .. (23.83,6) -- (193.17,6) .. controls (197.77,6) and (201.5,9.73) .. (201.5,14.33) -- (201.5,90.67) .. controls (201.5,95.27) and (197.77,99) .. (193.17,99) -- (23.83,99) .. controls (19.23,99) and (15.5,95.27) .. (15.5,90.67) -- cycle ;
%Up Down Arrow [id:dp4246149856363397] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (311.5,111) -- (328.25,102) -- (345,111) -- (335,111) -- (335,122) -- (345,122) -- (328.25,131) -- (311.5,122) -- (321.5,122) -- (321.5,111) -- cycle ;
%Image [id:dp05773900655841713] 
\draw (551.86,60.5) node  {\includegraphics[width=79.28pt,height=47.25pt]{imgs/aqua.jpg}};
%Rounded Rect [id:dp8230713593534384] 
\draw   (473.17,14.33) .. controls (473.17,9.73) and (476.9,6) .. (481.5,6) -- (618.17,6) .. controls (622.77,6) and (626.5,9.73) .. (626.5,14.33) -- (626.5,90.67) .. controls (626.5,95.27) and (622.77,99) .. (618.17,99) -- (481.5,99) .. controls (476.9,99) and (473.17,95.27) .. (473.17,90.67) -- cycle ;
%Rounded Rect [id:dp8551143788810873] 
\draw   (277.17,14.33) .. controls (277.17,9.73) and (280.9,6) .. (285.5,6) -- (380.83,6) .. controls (385.44,6) and (389.17,9.73) .. (389.17,14.33) -- (389.17,90.67) .. controls (389.17,95.27) and (385.44,99) .. (380.83,99) -- (285.5,99) .. controls (280.9,99) and (277.17,95.27) .. (277.17,90.67) -- cycle ;
%Right Arrow [id:dp3117459154120561] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (401.75,50.25) -- (443.5,50.25) -- (443.5,45) -- (459.5,55.5) -- (443.5,66) -- (443.5,60.75) -- (401.75,60.75) -- cycle ;
%Right Arrow [id:dp8603749881772891] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (211.17,51.25) -- (251.65,51.25) -- (251.65,46) -- (267.17,56.5) -- (251.65,67) -- (251.65,61.75) -- (211.17,61.75) -- cycle ;

% Text Node
\draw (293,30.38) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{53.00810800000001pt}\setlength\topsep{0pt}
\begin{center}
Obstacle\\Avoidance \\Module
\end{center}

\end{minipage}};
% Text Node
\draw (200.7,230.34) node [anchor=north west][inner sep=0.75pt]  [rotate=-318.34] [align=left] {{\scriptsize Disparity}\\{\scriptsize Calculation}};
% Text Node
\draw (201.67,302) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Instance}\\{\scriptsize Segmentation}};
% Text Node
\draw (351,245) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Combine}};
% Text Node
\draw (48,249) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Rectification}};
% Text Node
\draw (204.67,172) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize \textcolor[rgb]{0,0.01,1}{\textbf{Input}}}};
% Text Node
\draw (22,146) node [anchor=north west][inner sep=0.75pt]   [align=left] {Instance Segmentation with Depth Information};
% Text Node
\draw (64.49,14) node [anchor=north west][inner sep=0.75pt]   [align=left] {Stereo Images};
% Text Node
\draw (26,116) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large SOAR}};
% Text Node
\draw (526.49,10) node [anchor=north west][inner sep=0.75pt]   [align=left] {Robot};


\end{tikzpicture}

\caption{Illustration of our pipeline to decide where to explore from a pair of stereo images. Input is marked with ``blue'' color.}
\label{fig:pipeline}
\vspace{-4mm}
\end{figure}


==> tables/interest_weights.tex <==
\begin{table}
    \caption{The interest weights our system used for each class when choosing interesting locations to explore. The different values were arbitrarily chosen in order to observe whether the algorithm's decisions were made as expected.}
\centering
    \begin{tabular}{c|c}
    Class & Interest Weight \\
    \hline\hline 
    Person & 1.0 \\
    Chair & 0.5 \\
    Sports Ball & 0 \\
    Diver & 1.0 \\
    Robot & 0.5 \\
    \end{tabular}

    \label{tab:interest}
    \vspace{-4mm}
\end{table}


==> tables/results.tex <==
\newcommand{\addpic}{\includegraphics[width=15.3em]{example-image}}
\newcolumntype{C}{>{\centering\arraybackslash}m{15.3em}}
\setlength\tabcolsep{1pt} % default value: 6pt
\vspace{25mm}
\begin{table*}[hbt!]
% \caption{Selected results from the collected data. Col1: RGB image from the left camera, Col2:  Instance segmentation overlaid on the depth image, Col3: Visualization of how different safety buffers can be applied based on the class of objects (\textit{e.g., } we have no buffers for the sports balls and have larger buffers for people). For the first 3 cases, depth images are converted into gray scale for visual presentation, Col4: Demonstration of center heuristic (C) and interesting view heuristic (I) exploration decisions.}
\begin{tabular}{l*5{C}@{}}
\toprule
& RGB Image from the left camera & Instance Segmentation & With Safety Buffers{*} & Exploration Decisions\\ 
% & Left RGB & Depth Estimation & Instance Segmentation & With Buffers & Exploration Decisions\\ 
\midrule % \includegraphics[width=15.3em]{} 
1 & \includegraphics[width=15.3em]{resultsimgs/rgbcolor0.jpg}
& \includegraphics[width=15.3em]{resultsimgs/segcolor0.png}
& \includegraphics[width=15.3em]{resultsimgs/ground_000_buffer.jpg} 
&\includegraphics[width=15.3em]{resultsimgs/kjj_targetsrgb0.jpg} \\ 
2 & \includegraphics[width=15.3em]{resultsimgs/rgbcolor2.jpg}
& \includegraphics[width=15.3em]{resultsimgs/segcolor2.png}
& \includegraphics[width=15.3em]{resultsimgs/ground_002_buffer.jpg} 
& \includegraphics[width=15.3em]{resultsimgs/jjc_targetsrgb2.jpg}
\\ 
3 & \includegraphics[width=15.3em]{resultsimgs/rgbcolor17.jpg} 
& \includegraphics[width=15.3em]{resultsimgs/segcolor17.png}
& \includegraphics[width=15.3em]{resultsimgs/ground_017_buffer.jpg} 
& \includegraphics[width=15.3em]{resultsimgs/bcj_targetsrgb17.jpg}
\\ 
\midrule
4 & \includegraphics[width=15.3em]{resultsimgs/frame000510.png}
  & \includegraphics[width=15.3em]{resultsimgs/pool2_inst_left_00510.png}
  & \includegraphics[width=15.3em]{resultsimgs/masked_510_buffer.jpg}
  & \includegraphics[width=15.3em]{resultsimgs/pool2_targetsrgb00510.jpg} 
  \\
% 5 & 
%   & \includegraphics[width=12em]{resultsimgs/pool2_inst_left_00541.png}
%   &
%   & \includegraphics[width=12em]{resultsimgs/pool2_targetsrgb00541.jpg} 
%   \\ 
5 & \includegraphics[width=15.3em]{resultsimgs/frame000003.png}
  & \includegraphics[width=15.3em]{resultsimgs/pool7_inst_left_00003.png}
  & \includegraphics[width=15.3em]{resultsimgs/masked_003_buffer.jpg}
  & \includegraphics[width=15.3em]{resultsimgs/pool7_targetsrgb00003.jpg} 
  \\
6 & \includegraphics[width=15.3em]{resultsimgs/frame000476.png}
  & \includegraphics[width=15.3em]{resultsimgs/pool11_inst_left_00476.png}
  & \includegraphics[width=15.3em]{resultsimgs/masked_476_buffer.jpg}
  & \includegraphics[width=15.3em]{resultsimgs/pool11_targetsrgb00476.jpg} 
  \\
\bottomrule 
\end{tabular} 
\caption{Selected results from the collected data. Col1: RGB image from the left camera, Col2:  Instance segmentation overlaid on the depth image, Col3: Visualization of how different safety buffers can be applied based on the class of objects (\textit{e.g., } we have no buffers for the sports balls and have larger buffers for people). For the first 3 cases, depth images are converted into gray scale for visual presentation, Col4: Demonstration of center heuristic (C) and interesting view heuristic (I) exploration decisions.}
\label{tab:results}
\vspace*{-1mm}

\end{table*} 

==> tables/traing_res.tex <==
% "box": {"all": 65.12, "50": 88.71, "55": 88.71, "60": 87.18, "65": 85.67, "70": 79.05, "75": 74.6, "80": 65.91, "85": 47.67, "90": 30.71, "95": 2.97}, 
% "mask": {"all": 68.21, "50": 91.11, "55": 91.1, "60": 90.51, "65": 87.79, "70": 85.23, "75": 78.37, "80": 70.07, "85": 55.61, "90": 26.59, "95": 5.73}}, 
\setlength\tabcolsep{11.7pt} % default value: 6pt
\begin{table*}[ht!]
%\caption{YOLACT instance segmentation results on the SUIM test dataset}
\begin{tabular}{c ccccccccccc}
\toprule
& mAP All& .50 & .55 & .60 & .65 & .70& .75&.80 & .85 & .90 &.95 \\ 
% & Left RGB & Depth Estimation & Instance Segmentation & With Buffers & Exploration Decisions\\ 
\midrule % \includegraphics[width=15.3em]{} 
Box &  67.29 & 89.11& 89.11& 88.29& 87.02& 79.89& 74.39 &66.68 & 59.19 &35.84 & 3.32\\
Mask &  67.15& 90.33 & 90.33 & 90.33 & 86.5 &83.4 & 79.62 & 65.04 & 53.9 & 25.42 & 6.62 \\
\bottomrule 
\end{tabular}
\caption{YOLACT instance segmentation results on the SUIM test dataset}
\label{tab:yolact}
\vspace*{-5mm}
\end{table*} 
% \vspace*{-5mm}

% {"type": "val", "session": 20, "data": {"elapsed": 4.379734516143799, "epoch": 4678, "iter": 262024, "box": {"all": 67.29, "50": 89.11, "55": 89.11, "60": 88.29, "65": 87.02, "70": 79.89, "75": 74.39, "80": 66.68, "85": 59.19, "90": 35.84, "95": 3.32}, "mask": {"all": 67.15, "50": 90.33, "55": 90.33, "60": 90.33, "65": 86.5, "70": 83.4, "75": 79.62, "80": 65.04, "85": 53.9, "90": 25.42, "95": 6.62}}, "time": 1582011092.7009735}

==> tex/3_method_old.tex <==
% \input{figs/pipelinenew2}
\input{figs/soarlabel}
\section{METHODOLOGY}
\label{sec:methodology}
The proposed approach incorporates both instance segmentation and depth information to intelligently avoid obstacles in unstructured or dynamic environments, with the goal to optimize robot paths (\eg in terms of distance traveled, energy spent, and time taken) without compromising obstacle avoidance capabilities. The system obtains object labels and pixel locations from instance segmentation and fuses the information with depth information to assign clearance distances to obstacles. % objects are obstacles that need to be avoided. 

%The system can be instructed to avoid some classes of obstacles more than others, and it can also be instructed to ignore certain classes of obstacles.

% The system can also use the instance segmentation information to make decisions about how to explore the environment. Our approach assigns different berths to each object class and makes navigation decisions with the goal of exploring areas of the environment while minimizing the travel time.

\subsection{Information Fusion using a Stereo Camera}
We use a stereo camera as our only sensor to acquire (1) pixel-level masks and labels of each object using instance segmentation, and (2) depth information. Once both are acquired, we fuse them to provide semantic information to an obstacle avoidance module (see Fig.~\ref{fig:pipeline}).

\subsubsection{Instance Segmentation with Transfer Learning}\label{sec:insseg}
We choose YOLACT~\cite{bolya2019yolact} as the base instance segmentation module due to its real-time inference and competitive accuracy. We use ResNet50-FPN as a backbone network for achieving maximum inference speed since robots are likely to use low-power computation units (\eg an Nvidia Jetson TX2) to perform semantic inference. We collect a total of $2,263$ images, of which $1,682$ are labeled with \textit{diver}, \textit{robot}, and \textit{fin} (\ie diver's flippers) classes. Examples of labeled training images are shown in Fig.~\ref{fig:soarlabel}. The annotation was completed by volunteers with the Supervisely~\cite{supervisely} tool. In addition, we use $581$ images from the SUIM dataset~\cite{SUIM} which has \textit{diver}, \textit{fish}, and \textit{robot} classes. We refine a pre-trained YOLACT model, initially trained with the MS COCO dataset~\cite{lin2014microsoft}, with this additional data.

% 581 images for transfer learning
\subsubsection{Depth Estimation}
Our depth estimation process is as follows: %OpenCV~\cite{opencv_library} is used for  
\begin{enumerate}
\item We perform stereo rectification to obtain a transform matrix $\mathbf{R}$, projection matrix $\mathbf{P}$, and disparity-to-depth mapping matrix $\mathbf{Q}$ for each camera using a camera matrix $\mathbf{K}$ and distortion parameters $\mathbf{D}$ from each camera, a rotation matrix $\mathbf{R}$ between the first camera coordinate and the second camera coordinate, and a translation vector $\mathbf{T}$ between two cameras.
\item Next, we remove distortion from each image using the $\mathbf{K}$,  $\mathbf{D}$, $\mathbf{R}$, and $\mathbf{P}$ matrices.
\item After rectifying each pair of images, we run stereo matching to generate a disparity map.
\item Lastly, we estimate the depth information from the disparity map using $\mathbf{Q}$. 
% disparity using stereo matching (StereoSGBM\_create)
% generating depth map (reprojectImageTo3D)
\end{enumerate}

% \input{algs/alg1}
\input{tables/results1}
% \input{tables/result0}

\subsection{Obstacle Avoidance} %and Active Exploration}
Our obstacle avoidance algorithm is inspired be the Artificial Potential Field (APF) method~\cite{khatib1986real}. APF uses an attractive potential $f_a$ to guide the robot toward the goal and a repulsive potential $f_r$ to push the robot away from obstacles. The attractive potential is calculated as: %shown in Eq. \ref{eq:fa} and \ref{eq:fr}. 

\begin{equation} \label{eq:fa}
    f_a(x) = c(|x - x_g|)^2
\end{equation}

Here $c$ is a scaling constant, $x$ is the current robot position, and $x_g$ is the goal position. The repulsive potential is calculated as
\begin{equation} \label{eq:fr}
f_r(x) = 
\begin{cases}
    \eta(\frac{1}{p(x)} - \frac{1}{d_0})^2 & \text{if $p(x) \leq d_0$} \\ 
                                      0 & \text{if $p(x) > d_0$}
\end{cases}
\end{equation}

where $\eta$ is a constant, $p(x)$ is the closest obstacle to the position $x$, and $d_0$ is the largest distance from the obstacle at which the robot can sense the obstacle's repulsive force. In our case, we update $d_0$ based on semantic information about the obstacles. For instance, we assign $d_0 = 0$ for objects we can ignore (\eg bubbles or sports balls) while assigning a larger value for the objects (\eg coral reef, robots, people) we intend to avoid. In our implementation, the robot attempts to align its direction of motion with the attractive artificial potential field. It moves with a constant velocity and slows down when it is a certain distance away from the goal position.

% Note that the value of $d_0$ varies depending on what type of obstacle it is associated with. Namely, small or harmless objects such as sports balls or bubbles may have a small $d_0$, while bigger objects like animals or people have a larger $d_0$. 

% our predefined ``type of objects: distance'' dictionary
% We used a simple control strategy; 

% However, we observed that the robot did not maintain a consistent distance of $d_0$ from obstacles during our tests.
% % However, during our tests, sometimes the robot passed closer to obstacles than the intended distance $d_0$. 
% Instead, it began to turn away from obstacles as the repulsive field overcame the attractive field, but it sometimes passed too close to them, or even clipped them on its way to the goal. 

% % However, we observed that the robot did not maintain a consistent distance of $d_0$ from obstacles. During our tests, sometimes the robot passed closer to the obstacles than intended. To solve this problem, we implemented a strategy designed to intentionally maintain a distance of $d_0$ from obstacles; in particular, the robot is attracted to a path along a circle of radius $d_0$ around obstacles. 
% This is implemented as follows. The attractive gradient in the original APF is replaced by a unit vector $A$ that points from the robot to the goal. As long as we are at leasthttps://www.overleaf.com/project/5f99b4e90b42e20001f5be07 $d_0$ from the closest obstacle we will simply follow $A$. However, more work is required when we reach a distance of $d_0$ from an obstacle.

Our implementation, unlike traditional APF, enforces the rule that the robot must not come within $d_0$ of any obstacle. The robot, however, may face challenges maintaining fixed distances (\ie $d_0$) consistently from obstacles. Errors in state estimation, external forces such as wave effects for underwater robots, and wind for aerial drones may make it difficult to correctly keep such distances. We define a vector $\hat{v}$ in Eq~\ref{eq:v} that drives the robot to the goal based on the distance from the robot to the obstacle.

\begin{equation}\label{eq:v}
    \hat{v} = 
\begin{cases}
    \hat{a} & \text{if $x_o - x > d_0$} \\ 
    \hat{a} + c_1c_2\hat{r} & \text{if $x_o - x \leq d_0$}
\end{cases}
\end{equation}

% \input{figs/alg1}
% \input{figs/alg2}

% To account for this, we adopt a strategy so that the robot is attracted to a path along a circle of radius $d_0$ around obstacles, and if the robot gets too close to the obstacle, the obstacle's repulsive potential is increased to move the robot away.
We achieve this by creating a unit vector, $\hat{a}$, that points from the robot towards the goal, and another unit vector, $\hat{r}$, that points from the robot to the obstacle. As long as the robot is at least $d_0$ from the closest obstacle, the robot will simply follow $\hat{a}$. If the robot moves within a distance of $d_0$ from an obstacle, we use the unit vector $\hat{r}$, pointing from the robot to the obstacle. We multiply $\hat{r}$ by the factor $c_1$, given by: 

\begin{equation} \label{eq:c1}
    c_1 = -\hat{a} \cdot \hat{r}    
\end{equation}

Now, $c_1\hat{r} = -\text{proj}_{\hat{a}}\hat{r}$. Adding $c_1\hat{r}$ to $\hat{a}$ removes the component of $\hat{a}$ parallel to $\hat{r}$. This means that the sum $\hat{a} + c_1\hat{r}$ is perpendicular to $\hat{r}$:
\begin{equation} \label{eq:perp}
    (\hat{a} - (\hat{a} \cdot \hat{r})\hat{r} ) \cdot \hat{r} = \hat{a} \cdot \hat{r} - \hat{a} \cdot \hat{r} = 0 
\end{equation}
 
If the robot is at a distance $d_0$ from an obstacle, then $\hat{a} + c_1\hat{r}$ causes the robot to attempt to avoid the obstacle at a consistent radius $d_0$ while still moving towards the goal.

However, due to the momentum and limits on turning speed, the robot may still come closer than $d_0$ to an obstacle. If the robot does move closer than $d_0$ to the obstacle, we use the additional factor $c_2$ to scale the repulsive component $c_1\hat{r}$ to course-correct the robot's path away from the obstacle.
\begin{equation} \label{eq:c2}
    c_2 = \frac{1 - b}{d_0}|x_o-x| + b     
\end{equation}

Here, $x_o$ is the obstacle position, $x$ is the robot position, and $b$ is a constant greater than 1 that represents the maximum value $c_1\hat{r}$ can be scaled by. $c_2$ scales inversely from the robot's distance to the obstacle, and obtains a value between $1$ and $b$ as we approach the obstacle.

Thus, our calculation of the robot's direction of movement $\hat{v}$ at any given point can be summarized by:

\begin{equation}
    \hat{v} = 
\begin{cases}
    \hat{a} & \text{if $x_o - x > d_0$} \\ 
    \hat{a} + c_1c_2\hat{r} & \text{if $x_o - x \leq d_0$}
\end{cases}
\end{equation}


% There is at least one problem with this approach: Since we only calculate the potential from the closest obstacle, some other obstacle farther away from the robot with a large enough $d_0$ might go unnoticed by the robot, resulting in the robot approaching closer to the farther obstacle than intended. This is probably an edge case in practice. 

==> tex/7_ack.tex <==
\section*{ACKNOWLEDGMENT}
